Scale-Agnostic Super-Resolution in MRI using Feature-Based Coordinate Networks

We propose using a coordinate network decoder for the task of super-resolution in MRI. The continuous signal representation of coordinate networks enables this approach to be scale-agnostic, i.e. one can train over a continuous range of scales and subsequently query at arbitrary resolutions. Due to the difficulty of performing super-resolution on inherently noisy data, we analyze network behavior under multiple denoising strategies. Lastly we compare this method to a standard convolutional decoder using both quantitative metrics and a radiologist study implemented in Voxel, our newly developed tool for web-based evaluation of medical images.

==> figures/table_quant.tex <==
\setlength{\extrarowheight}{1pt}
% for options to add space b/w rows, see https://tex.stackexchange.com/questions/26690/how-to-add-extra-spaces-between-rows-in-tabular-environment
\setlength{\tabcolsep}{4pt} % spacing b/w cols, default 6pt

\begin{table}[t]
\floatconts
  {tab:example}%
  {\caption{sketch latex for screenshot}}%
  {\begin{tabular}{|c|lccc|ccc|}
  \toprule
  \hline
  & & & \textbf{Scale-} & \textbf{Train}& \multicolumn{3}{c}{\textbf{Query scale} (VIF/PSNR)} \\
  & \textbf{Method} & $\boldsymbol{\lambda}$& \textbf{agnostic} & \textbf{scale} & 1.5$\times$ & 2$\times$ & 3$\times$ \\ \hline
  \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Default}}} & Bicubic & --- & \ding{51} & ---  & .87/34.2 & .79/31.4 & .64/27.6\\
  & \Coord & 10 & \ding{51} & 1-2$\times$      & .92/33.8 & .87/31.0 & .76/26.9\\
  & \Conv   & 0 & & 2$\times$  & ---  & .82/32.3 & --- \\ %[1mm]
  \hline
  \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Ablation}}} & 
  \Coord & 0 & \ding{51} & 1-2$\times$ & .95/33.0  & .88/30.2 &  .74/26.3 \\
  & \Coord    & 10 & \ding{51} & 2$\times$       & .95/33.2 & .90/30.4 &  .77/26.2 \\
  & \Conv & 10 & & 2$\times$       & ---       & .81/32.2 & --- \\
  \hline
\end{tabular}}
\end{table}

==> figures/table_reader_study.tex <==
\setlength{\extrarowheight}{0pt}
% for options to add space b/w rows, see https://tex.stackexchange.com/questions/26690/how-to-add-extra-spaces-between-rows-in-tabular-environment
\setlength{\tabcolsep}{3pt} % spacing b/w cols, default 6pt

\setlength{\tabcolsep}{2pt} % spacing b/w cols, default 6pt
\begin{table}[t]
\floatconts
  {tab:example}%
  {\caption{sketch latex for screenshot}}%
  {\begin{tabular}{|c|l|}
  \toprule
  \hline
  \textbf{Score} & \textbf{Criteria} \\
  \hline
  +/-2 & Coord:~\textit{much} better/worse \\
  +/-1 & Coord:~\textit{slightly} better/worse \\
  0 & Coord, conv: no difference \\
  \hline
\end{tabular}}
\end{table}

\setlength{\tabcolsep}{6pt} % spacing b/w cols, default 6pt
\begin{table}[t]
\floatconts
  {tab:example}%
  {\caption{sketch latex for screenshot}}%
  {\begin{tabular}{|c|cc|}
  \toprule
  \hline
%   & \multicolumn{2}{c}{Reader} \\
  \textbf{Reader} & \textbf{Noise} & \textbf{Sharpness}\\
  \hline 
  1     &\color{white}\colorbox{rcn}{.70 $\pm$ .64}
        &\color{white}\colorbox{rcs}{1.4 $\pm$ .69} \\
  2     &\color{white}\colorbox{rrn}{.78 $\pm$ .46}
        &\color{white}\colorbox{rrs}{.02 $\pm$ .14} \\
  Pooled  &\color{white}\colorbox{rcrn}{.74 $\pm$ .56}
        &\color{white}\colorbox{rcrs}{.70 $\pm$ .84} \\
  \hline
\end{tabular}}
\end{table}

==> figures/voxel.tex <==
\begin{figure}[b!]%[htbp]
\centering
  \includegraphics[width=0.8\textwidth]{figures/voxel.png}
  \caption{User interface for Voxel, our web-based tool used in the radiologist reader study}
  \label{fig:voxel}
\end{figure}
